An Argumentative Dialogue System for COVID-19 Vaccine Information

Dialogue systems are widely used in AI to support timely and interactive communication with users. We propose a general-purpose dialogue system architecture that leverages computational argumentation to perform reasoning and provide consistent and explainable answers. We illustrate the system using a COVID-19 vaccine information case study.

==> s_argumentation.tex <==
%\textcolor{red}{COPIAINCOLLATO, DA RISCRIVERE}
%In this section we recall the basics of abstract argumentation.
Abstract Argumentation (AA)~\cite{Dung95} is a branch of Artificial Intelligence (AI) that gained significant attention in the last years due to its capability of modelling debates, dialogues, and, in general, situations where conflicts and diversity of opinions arise. One important point that leads to the usage of AA as reasoning mechanism at the core of several dialogue-based applications in AI is also its natural aptitude to provide “explanations”. In fact, in recent years, the capability of providing motivations for systems/agents’ behaviours has become crucial in AI, and AA is taking on a more and more central role. In fact, modelling a dispute/dialogue as an AA framework not only offers the possibility of locating the arguments that represent a good/bad point in a rebuttal, but has the further advantage of possibly providing a “witness” of the reason why a certain argument is a good/bad point. From a technical standpoint, the disputes in AA are modelled as graphs, where the arguments, that are the sentences claimed by the agents participating the dispute, are the nodes, and the conflicts/contradictions between the sentences, named attacks, are the edges of the graph. As an example, consider the following scenario. Andrea says argument $a$: “Milan is a very livable city”. Matt says argument $b$: “Milan is one of the most polluted cities of the world, so it is absolutely not livable”. Alice says argument $c$: “Several parameters are used to establish whether a city is livable, thus you can’t say that Milan is not livable”. This scenario can be modelled as the AA graph $\langle A, D\rangle$, where $A$ consists of the arguments $a,b, c$ and $D$ consists of the edges $(a,b), (b,a), (c,b)$.

A lot of work has been devoted to reason over the argumentation graph~\cite{Baroni2009,FazzingaFF19,CharwatDGWW15}, and several ways of identifying “robust” arguments or sets of arguments have been proposed, called semantics~\cite{Dung95,Dung2007}. Among others, one of the most used semantics is the admissible one, that establishes that a set $S$ of arguments is an admissible extension (that is, it conforms to the admissible semantics) if and only if i) $S$ is conflict-free, i.e. there is no attack between arguments in $S$ and ii)$S$ attacks every argument (outside $S$) attacking arguments in $S$. Condition ii) reveals that the admissible semantics is based on the fundamental concept of defense: to be an admissible extension, $S$ must defend every argument $a \in S$, that is $S$ must counterattack every attack from outside towards $a$.   Continuing the above example, both $S_1=\{c\}$ and $S_2=\{a,c\}$ are admissible extensions, while  $S_3=\{a,b\}$ and $S_4=\{b,c\}$  are not, as they are not conflict-free, and neither is $S_5=\{b\}$ as it does not defend itself against the attack from $c$. 
%
\textcolor{red}{As regard single arguments, the most important notion is the \emph{acceptance} condition: an argument $a$ is \emph{acceptable} in a set $S$ iff $S$ defends $a$ from every attack towards $a$.}

==> s_framework.tex <==
%In order to explain the workings of our dialog system, we shall introduce relevant definitions.
We are now ready to detail the components of our dialogue system.

\subsection{Knowledge Representation and Reasoning}

Our \textit{background knowledge} is expressed as an argument graph.

\begin{definition}[Argumentation graph]
\textcolor{red}{An argumentation graph is a tuple $\langle A,R,D,T \rangle$, where $A$ and $R$ are the arguments of the graph and are called \emph{status} arguments and \emph{reply} arguments, respectively, $D \subseteq A\times A$ encodes the attack/defeat relation, and $T \subseteq A\times R$ encodes the support relation.}
\end{definition}

Each argument in $A$ is annotated with a set of natural language sentences, as described in the previous section.
We say that $a$ \emph{attacks} (resp., \emph{supports}) a reply node $r$ iff $(a,r) \in D$ (resp., $(a,r) \in T$). By extension, we say that a set $S$ attacks (resp., supports) $r$, or equivalently that $r$ is attacked by (resp., supported by) $S$, iff there exists an argument $a \in S$ s.t. $a$ attacks (resp., supports) $r$.

In addition to the background knowledge, each dialogue sessions relies on \textit{dynamically acquired knowledge}, expressed as a set of facts or \textit{status arguments} $S$.
The dialogue strategy is to provide the user with a reply that is supported and defended by $S$. However, differently from other proposals, our system does not simply select a consistent reply at each turn. On the contrary, it strategizes in order to provide only robust replies, possibly delaying replies that need further fact-checking. To that end, the two following definitions distinguish between \emph{consistent} and \emph{potentially consistent} reply. The former can be given to the user right away, as it 
%is already proven that it 
can not possibly be proven wrong in the future.\footnote{ The implicit assumption here is that the user does not enter conflicting information, and that the language model correctly interprets the user input. Clearly, if this is not the case, the system's output becomes unreliable. But that wouldn't depend on the underlying reasoning framework. The definition of fall-back strategies able to handle such exceptions would be an important extension to the system.}
%\textcolor{magenta}{PT: Mi sembra forte. Anche se l'utente stesso si contraddice in futuro? mettere qc del tipo: unless, of course, future user input contradicts the input provided by the user so far.}
The latter, albeit consistent with the current known facts, may still be defeated by future user input, and therefore it should be delayed until a successful elicitation process is completed.
%for what the process of enforcement is needed.   
The formal definitions are based on the KB and on a representation of the state of the dialogue consisting of two sets: $S$ and $N$. In particular, $S\subseteq A$ contains the arguments activated during the conversation so far, whereas $N\subseteq S$ contains arguments in support of the system's possible replies to the user.

\begin{definition}[Consistent reply]
\label{def:ar}
Given an argumentation graph $\langle A,R,D,T \rangle$ and two sets $S\subseteq A$ and $N\subseteq S$, a  reply $r\in R$ is \emph{consistent} iff $N$ supports $r$ and $r$  is acceptable in $S$.  
\end{definition}

\begin{definition}[Potentially consistent reply]
\label{def:pr}
Given an argumentation graph $\langle A,R,D,T \rangle$ and two sets $S\subseteq A$ and $N\subseteq S$, a  reply $r\in R$ is \emph{potentially consistent} iff $N$ supports $r$, $S$ does not attack $r$ and $r$  is not acceptable in $S$.  
\end{definition}

Finally, users can challenge the system output. An \emph{explanation} of a reply $r$ consists of two parts. The first one contains the arguments leading to $r$, i.e., those belonging to a set $S$ that supports $r$. The second one encodes the \textit{why not}s, to explain why the chatbot did not give other replies. %due to  the fact that they were attacked by $S$.

\begin{definition}[Explanation]
\label{def:expl}
Given an argumentation graph $\langle A,R,D,T \rangle$, a set $S\subseteq A$ and a  reply $r\in R$, an \emph{explanation} for $r$ is a pair $\langle Supp, NotGiven\rangle$, where $Supp$ contains the arguments $a \in S$ s.t. $(a,r) \in T$ and $NotGiven$ is a set of pairs $\langle r',N' \rangle$, where $r'\neq r$, $r'$ is supported by $S$ and $N'\subseteq S$ contains the arguments $b$ attacking $r'$.  
\end{definition}
%\textcolor{magenta}{$Supp$ contiene tutti gli argomenti a supporto o basta uno? $NotGiven$ contiene tutte le coppie che si possono fare o solo alcune? (direi tutte?) $N'$ contiene tutti gli attacchi o solo uno? (forse basta uno?)}


\subsection{Dialogue System Routine}

%Our approach works as described in 
The behaviour of our dialogue system is specified by Algorithm \ref{algo}.

At line \ref{line:start} the system starts the conversation with the user. This procedure includes the understanding of what is the question of the user and therefore which will be the context of the reasoning.
In this work we will not focus on how this method is implemented, but rather on how to collect the relevant information and how to provide the correct answer.
%
At line \ref{line:acquire1}, the first user sentence is acquired and stored into variable $U$.
Lines \ref{line:init1}-\ref{line:init2} initialize the set
$S$ that will be used to store the arguments activated during the conversation, and variable $r$ that will be used to
store the current reply to be given to the user.
%, respectively.

\begin{algorithm}[h!]
\caption{Dialogue System}
\begin{algorithmic}[1]
\label{algo}
%\REQUIRE{a set $Q$ of KB nodes}
%\ENSURE{a set $X$ of KB nodes}
\STATE{\textsf{startConversation}()} \label{line:start}
\STATE{$U\leftarrow$ \textsf{acquireUserSentence}()} \label{line:acquire1}
\STATE{$S\leftarrow \emptyset$}\label{line:init1}
\STATE{$r\leftarrow$ NULL}\label{line:init2}
\WHILE{$U$ is not a stop sentence} \label{line:while1}
\IF{$U$ is not an explanation request} \label{line:if}
\STATE{$N\leftarrow$ \textsf{computeMatches}($U$)} \label{line:sanitize1}
\STATE{$S\leftarrow S\cup N$} \label{line:updateS1}
\STATE{$\langle Cons,PCons\rangle\leftarrow$ \textsf{retrieveReplies}($S,N$)}\label{line:retrieve1}
\STATE{\textit{reply} $\leftarrow$ FALSE} \label{line:initReply}
\WHILE{\textit{reply} is FALSE} \label{line:while2}
	\IF{$Cons \neq \emptyset$}\label{line:ifAdm}
		\STATE{$r\leftarrow$ \textsf{selectCandidateReply}($Cons$)} \label{line:select1}
		\STATE{\textsf{replyToTheUser}($r$)}\label{line:reply1}
		\STATE{\textit{reply} $\leftarrow$ TRUE}
	\ELSE	
		\IF{$PCons = \emptyset$}\label{line:ifPAdmEmpty}
		\STATE{\textsf{terminateConversation}()}
		\ENDIF
		\STATE{$r \leftarrow$ \textsf{selectCandidateReply}($PCons$)}\label{line:select2}
		\STATE{$N^*\leftarrow$ \textsf{selectDefenceNodes}($r$)}\label{line:defence}
		\STATE{$N^{new}\leftarrow\emptyset$}
	\FORALL{$n \in N^*$} \label{line:for}
	\STATE{\textsf{replyToTheUser}($n$)} \label{line:reply2}
	\STATE{$U\leftarrow$ \textsf{acquireUserSentence}()} \label{line:acquire2}
	\STATE{$N\leftarrow$ \textsf{computeMatches}($U$)} \label{line:sanitize2}
	\STATE{$N^{new}\leftarrow N^{new}\cup N$} \label{line:endfor}
	%\STATE{$S=S \cup Q$}
	\ENDFOR
		\STATE{$S\leftarrow S \cup N^{new}$}
	\IF{ $r$ is a consistent reply w.r.t $S$}\label{line:acc}
		\STATE{\textsf{replyToTheUser}($r$)}
		\STATE{\textit{reply} $\leftarrow$ TRUE}
	\ELSE
	\STATE{$\langle Cons,PCons\rangle\leftarrow$ \textsf{retrieveReplies}($S, N^{new}$)} \label{line:retrieve2}
	\ENDIF
	\ENDIF
	\ENDWHILE
	\ELSE 
	\STATE{$Expl\leftarrow$ \textsf{retrieveExplanation}($S,r$)}\label{line:retrieveExpl}
\STATE{\textsf{replyToTheUser}($Expl$)} \label{line:reply3}
\ENDIF
\STATE{$U\leftarrow$ \textsf{acquireUserSentence}()}
	\ENDWHILE
	\end{algorithmic}
\end{algorithm}


The outer \textbf{while} loop (line \ref{line:while1}) handles the conversation with the user, until they terminate the chat
by using a closing sentence. 
Line \ref{line:sanitize1} encodes the invocation of function 
\textsf{computeMatches}, 
%that deals with the removal of the personal information of the user and with matching 
which matches
the relevant information given by the user with the status arguments of the KB (see Section~\ref{sec:computeMatches}).
The output of function \textsf{computeMatches} is a set $N$ of status arguments, that are first added to $S$ (line \ref{line:updateS1}) and then given as input to function \textsf{retrieveReplies} 
in order to retrieve the reply arguments that are supported by $N$. In particular, the output of  \textsf{retrieveReplies} is a pair
$\langle Cons,PCons\rangle$, where $Cons$ is a set of consistent replies, that is, they are reply arguments
that are supported by $N$ and are acceptable w.r.t. $S$, according to Definition~\ref{def:ar}.
Instead, set $PCons$ contains the potentially consistent replies, that are reply arguments supported by $N$ that are not acceptable in $S$ at the moment, as per Definition~\ref{def:pr}. This basically means that an argument $a \in PCons$  could turn to be accepted in $S$ by collecting more information by the user. 
Then the operations aimed at finding a reply to be given to the user start.
In fact, the inner \textbf{while} loop (line \ref{line:while2}) stops when variable \emph{reply} becomes true.
%
If $Cons$ is not empty, %to provide the user with a consistent reply is sufficient to randomly select one 
a reply is arbitrarily selected among those in $Cons$ (line \ref{line:select1}) and returned to the user (\ref{line:reply1}).\footnote{This selection could be made by a more sophisticated strategy, but we leave this to future work}
%
In case both $Cons$ and $PCons$
are empty (line \ref{line:ifPAdmEmpty}), 
a consistent reply can not be found and the conversation is terminated. Otherwise, if $PCons$ is not empty,
Algorithm \ref{algo} starts the elicitation strategy, aimed to turn some reply in $PCons$ consistent. Specifically, a reply $r$ is selected from $PCons$ (line \ref{line:select2}) and the arguments not belonging to $S$ that defend $r$ from its attacks are retrieved (line \ref{line:defence}). Then, each of these arguments $n$ (line \ref{line:for}) is transformed in a proper sentence and  submitted to the user (line \ref{line:reply2}), to see if the user confirms or denies the information contained in $n$. The reply of the user to each $n$ is collected (line \ref{line:acquire2}) %, it is sanitized 
and the arguments activated by the reply are added to set $N^{new}$ (line \ref{line:endfor}). At the end of this process, $N^{new}$ eventually contains new arguments that, added to $S$, may cause $r$ to be a consistent reply. If this is the case (line \ref{line:acc}), $r$ is given to the user and the inner \textbf{while}  loop %at line \ref{line:while2} 
terminates,
otherwise new candidate replies are retrieved (line \ref{line:retrieve2}) and the %\textbf{while} 
loop continues with another iteration. 

%In the case that the \emph{if} at line \ref{line:if} is false,
\textcolor{red}{If $U$ is an explanation request (line \ref{line:if}), i.e., the user is looking for an explanation for the last reply $r$ the chatbot gave to them, the proper explanation, according to Definition~\ref{def:expl}, is retrieved at line \ref{line:retrieveExpl}, and given to the user (line \ref{line:reply3}).}

The following proposition states a property of consistent replies. Indeed, the fact that a reply $r$ is consistent w.r.t. $S$ means that $S$ contains a defence for every attack towards $r$, thus as the algorithm proceeds and $S$ grows, no status arguments added to $S$ can make $r$ inconsistent,
as long as $S$ remains conflict-free, i.e., as long as the user does not make conflicting statements. %\textcolor{magenta}{bisognerebbe dire secondo me che as $S$ resta conflict-free fintantoch\'e l'utente non si contraddice. (vero??). A ogni modo, bisognerebbe rendere questo risultato consistente con quanto affermato prima, cio\`e che a consistent reply ``can not be proven wrong in the future'' che forse va smorzato}

\begin{proposition}
 Given an argumentation graph $\langle A,R,D,T \rangle$ and a set $S \subseteq A$, a consistent reply $r$ w.r.t $S$ is a consistent reply for any conflict-free set $S' \supseteq S$.
\end{proposition}

%\noindent
Section \ref{sec:case} provides an example of how Algorithm \ref{algo} works.\\

\noindent
\textbf{Remark.} % on  Algorithm \ref{algo}:
Algorithm \ref{algo} assumes that,
for at least one of the candidate replies, some defence nodes exists (line \ref{line:defence}). %\textcolor{magenta}{non ho capito l'inglese: vuol dire at least one of the candidate replies has a defence node? inoltre cosa vuol dire defence node? non serve un attacco per avere una difesa? quali candidate replies si intendono? quelle che si vogliono fornire, o quelle per cui s vuole giustificare che sono state escluse?} 
The argumentation graph we built from the AIFA website for the case study of COVID-19 vaccines has a particular structure that verifies this assumption (see Section~\ref{sec:case}). In general, the retrieval and selection of defence nodes for arbitrary argumentation graphs requires a more complicated strategy, which we defer to future works.

\subsection{Language Module}

\label{sec:computeMatches}
The \textsf{computeMatches} function  (lines~\ref{line:sanitize1}, \ref{line:sanitize2}) analyzes the user input, compares it with the argument annotations in the KB, and returns the set of status arguments that correspond to the information entered by the user.

In particular, each argumentative node in the KB is annotated with a set of natural language sentences %that express the concept embodied by the node. 
representing some possible ways a user would express the fact it is meant to encode.
The language module compares the user input with such sentences, so as to select those similar enough to be considered matched, and enable the activation of the correct argumentative nodes.


To evaluate sentence similarity we resort to \textit{sentence embeddings}.
These are high-dimensional numerical representations of textual sentences that can be computed using (pre-trained) neural architectures.
Many embeddings have been proposed along the years~\cite{ELMO,glove}, and modern attention-based~\cite{attention} sentence embeddings such as BERT~\cite{BERT} do not only model the syntactic content and structure of a sentence, but also capture its meaning.
Ideally, if two sentences have a similar meaning, they will be mapped onto similar sentence embedding.
%
Sentence embeddings have been used successfully in a variety of NLP tasks, including hard ones such as understanding negations and speculations, and have shown to outperform traditional rule-based systems~\cite{info:doi/10.2196/18953}.


Among the many possible models, we have decided to focus on Sentence-BERT models~\cite{SBERT}, which are specifically trained to perform well on tasks of sentence similarity. While it is possible to train new models for specific domains or tasks, many pre-trained models are already available and can be used as off-the-shelf tools without the need of creating a corpus, nor to perform a training or fine-tuning steps.

The similarity between two embeddings can be computed using any similarity function that operates on high-dimensional numerical vectors. We use the Bray-Curtis similarity~\cite{braycurtis} since it has led to satisfactory results in previous works~\cite{cross-lingual}, but other measures, such as cosine similarity~\cite{cosine}, may be valid alternative.
A possible alternative to the use of sentence embeddings combined with a similarity measure may be the use of neural architectures specifically trained to perform this task, such as cross-encoders~\cite{SBERT}. However, the computational footprint of these techniques may be too heavy in most contexts, since they require to encode and process any possible pair at any step of iteration.

Given a measure of similarity between two sentences, we transform it to a Boolean value by applying a threshold, which is an hyper-parameter of the architecture. In this way, we discriminate between the pairs of sentences that are similar enough to be considered matched, and those that are not.

==> s_results.tex <==
%Our experiments are limited to the matching method and are intended as a preliminary evaluation 

To assess the effectiveness of our \textsf{computeMatches} method based on sentence embeddings and similarity measures,
we run a preliminary experimentation on a small-sized dataset built around the use case of vaccines for COVID-19.
%is capable of matching sentences that embodies a similar semantic meaning. 
We are especially interested in evaluating our method on sentences with a similar syntactic structure, but different meaning (e.g., a sentence and its negation).

We consider only 6 argumentative nodes that correspond to the presence and the absence of 3 particular medical conditions, i.e., celiac disease, immunosuppression, and drug allergy.
For each node, our knowledge base contains from 3 to 7 sentences that can be used to express the same concept (see Table~\ref{table:sentences}).
We compare these sentences between each other and use a threshold value on their similarity scores to discriminate between matched and not matched.
To evaluate our method quantitatively, we treat it as a binary classification task on every possible pair of (different) sentences. If the two sentences belong to the same argumentative node, their pair is considered a positive instance, otherwise it is considered negative.

In our experiment we compare different models of sentence embeddings and different threshold criteria.
For sentence embeddings we evaluate the following Sentence-BERT~\cite{SBERT} models:\footnote{All the implementations of the models are taken from \url{http://www.sbert.net/}.}
\begin{itemize}
    \item \texttt{stsb-mpnet}: based on MPNet~\cite{MPNet} and pre-trained for semantic similarity on the STSbenchmark~\cite{stsb}.
    \item \texttt{paraphrase-mpnet}: based on MPNet and pre-trained for paraphrase mining.
    \item \texttt{paraphrase-TinyBERT-L6}: based on TinyBERT~\cite{TinyBERT} and pre-trained  for paraphrase mining.
    \item \texttt{paraphrase-MiniLM-L3}: based on MiniLM~\cite{MiniLM} and pre-trained  for paraphrase mining.
    \item \texttt{nq-distilbert}: based on DistilBERT~\cite{DistilBERT} and pre-trained for question answering on Google’s Natural Questions dataset~\cite{googqa}.
    \item \texttt{paraphrase-multilingual-mpnet}: multilingual extension~\cite{DBLP:conf/emnlp/ReimersG20} of the monolingual model. We have decided to include this model in the perspective of future multi-lingual applications. 
\end{itemize}
%
We also include TF-IDF representation as in Charras et al.~\cite{embedding-chatbot}, Chalaguine and Hunter~\cite{Hunter}, using the entire set of sentences to create the vocabulary.
%
As thresholds, we use three fixed values (0.75, 0.70, 0.65), and two values that are based on the distribution of the similarity scores: one is given by the average of the similarities (mean), and the other one is given by the sum between the average similarity and the standard deviation (mean+std).


For each combination of models and thresholds, we measure precision, recall, and F1 score of the positive class (see Table~\ref{table:results}).
Precision is especially important: false positives can be seen as cases where the system ``misunderstands" the input of the user, and therefore precision can be seen as a measure of \emph{correctness}.
Recall instead can be see as a measure of the ability of the system to not ``miss" information contributed by the user.
For the purposes of our system, poor recall is a less serious problem than poor precision, since the argumentative reasoning module proactively asks the user for missing bits of information that would influence the final result.
In our perspective, the priority must be to guarantee the correctness of the final answer, even if this means that the system will, in some cases, ask for information that the user has already submitted. For this reason, we use precision as the main metric of comparison.

\begin{table}[!t]
\centering
 \caption{Experimental results of the embedding models and the threshold criterion on the sentence matching task.}
 \label{table:results}
 \begin{tabular}{l l c c c}
 \noalign{\smallskip}
 \hline
 \noalign{\smallskip}
  Embedding Model & Threshold &   P & R  & F1\\
 \noalign{\smallskip}
 \hline
 \noalign{\smallskip}
 \multirow{5}{*}{stsb-mpnet} 
&	mean	&	0.33	&	\textbf{1.00}	&	0.50	\\
&	mean+std	&	0.99	&	\textbf{1.00}	&	\textbf{0.99}	\\
&	0.75	&	\textbf{1.00}	&	0.67	&	0.80	\\
&	0.70	&	\textbf{1.00}	&	0.86	&	0.92	\\
&	0.65	&	\textbf{1.00}	&	0.97	&	\textbf{0.99}	\\

 \hline

 \multirow{5}{*}{paraphrase-mpnet} 
&	mean	&	0.32	&	\textbf{1.00}	&	0.49	\\
&	mean+std	&	0.99	&	\textbf{1.00}	&	\textbf{0.99}	\\
&	0.75	&	\textbf{1.00}	&	0.86	&	0.92	\\
&	0.70	&	\textbf{1.00}	&	0.94	&	0.97	\\
&	0.65	&	0.96	&	\textbf{1.00}	&	0.98	\\

 \hline

 \multirow{5}{*}{paraphrase-TinyBERT-L6~} 
&	mean	&	0.40	&	\textbf{1.00}	&	0.57	\\
&	mean+std	&	0.72	&	0.99	&	0.83	\\
&	0.75	&	\textbf{1.00}	&	0.46	&	0.63	\\
&	0.70	&	0.94	&	0.70	&	0.80	\\
&	0.65	&	0.81	&	0.94	&	0.87	\\

 \hline

 \multirow{5}{*}{paraphrase-MiniLM-L3} 
&	mean	&	0.43	&	\textbf{1.00}	&	0.60	\\
&	mean+std	&	0.55	&	0.96	&	0.70	\\
&	0.75	&	0.81	&	0.43	&	0.57	\\
&	0.70	&	0.66	&	0.61	&	0.63	\\
&	0.65	&	0.57	&	0.87	&	0.69	\\

% \hline

% \multirow{5}{*}{paraphrase-MiniLM-L12} 
% &	mean	&	0.43	&	\textbf{1.00}	&	0.60	\\
% &	mean+std	&	0.63	&   \textbf{1.00}	&	0.78	\\
% &	0.75	&	0.95	&	0.59	&	0.73	\\
% &	0.70	&	0.83	&	0.86	&	0.84	\\
% &	0.65	&	0.68	&	0.97	&	0.80 \\

 \hline

 \multirow{5}{*}{nq-distilbert} 
&	mean	&	0.37	&	\textbf{1.00}	&	0.54	\\
&	mean+std	&	0.50	&	0.75	&	0.60	\\
&	0.75	&	0.96	&	0.33	&	0.49	\\
&	0.70	&	0.64	&	0.46	&	0.54	\\
&	0.65	&	0.58	&	0.64	&	0.61	\\

 \hline


 \multirow{5}{*}{paraphrase-multilingual-mpnet ~~ }
 &	mean	&	0.31	&	\textbf{1.00}	&	0.47	\\
&	mean+std  ~~  &   0.99	&	0.97	&	0.98	\\
&	0.75	&	\textbf{1.00}	&	0.81	&	0.90	\\
&	0.70	&	0.98	&	0.93	&	0.96	\\
&	0.65	&	0.90	&	\textbf{1.00}	&	0.95	\\

 \hline


 \multirow{5}{*}{TF-IDF}
&	mean	&	0.27	&	0.71	&	0.39	\\
&	mean+std	&	0.34	&	0.39	&	0.36	\\
&	0.75	&	0.38	&	0.07	&	0.12	\\
&	0.70	&	0.33	&	0.07	&	0.12	\\
&	0.65	&	0.50	&	0.14	&	0.22	\\


\noalign{\smallskip}
 \hline
 \end{tabular}
\end{table}



\begin{table}[!t]
\centering
 \caption{Sentences used in our case study and the argumentative node they are associated with.}
 \label{table:sentences}
 \begin{tabular}{|c|c|l|}

 \hline

   Node ID ~&~ Sent. ID ~&   Sentence\\

 \hline

N1	&  S1 &	I am celiac \\
N1	&  S2 &	I suffer from the celiac disease \\
N1	&  S3 &	I am afflicted with the celiac disease \\
N1	&  S4 &	I have the celiac disease \\
N1	&  S5 &	I recently found out to be celiac \\
N1	&  S6 &	I have suffered from celiac disease since birth \\
 \hline
N2	& S7  &	I do not have the celiac disease \\
N2	&  S8 &	I am not celiac \\
N2	&  S9 &	I do not suffer from the celiac disease \\
N2	&  S10 &	I am not afflicted with the celiac disease \\
 \hline
N3	&  S11 &	I am not immunosuppressed \\
N3	&  S12 &	I do not suffer from immunosuppression \\
N3	&  S13 &	I am not afflicted with immunosuppression \\
 \hline
N4	&  S14 &	I am immunosuppressed \\
N4	&  S15 &	I suffer from immunosuppression \\
N4	&  S16 &	I am afflicted with immunosuppression \\
N4	&  S17 &	I do suffer from immunosuppression \\
N4	&  S18 &	I indeed suffer from immunosuppression \\
N4	&  S19 &	I recently found out to be immunosuppressed \phantom{kk}\\
 \hline
N5	&  S20 &	I do not have any drug allergy \\
N5	&  S21 &	I do not suffer from drug allergies \\
N5	&  S22 &	I do not suffer from any drug allergy \\
N5	&  S23 &	I am not afflicted with any drug allergy \\
N5	&  S24 &	I do not have medication allergies \\
N5	&  S25 &	I do not have any medication allergy \\
 \hline
N6	&  S26 &	I have a drug allergy \\
N6	&  S27 &	I do have a drug allergy \\
N6	&  S28 &	I have a serious drug allergy \\
N6	&  S29 &	I suffer from drug allergy \\
N6	&  S30 &	I am afflicted with drug allergies \\
N6	&  S31 &	I suffer from medication allergies \\

 \hline
 \end{tabular}
\end{table}





Our results clearly show that the \texttt{stsb-mpnet} and the \texttt{paraphrase-mpnet} models are the best ones, with the former achieving perfect precision with all the fixed similary scores and the latter achieving equivalent or even better F1 scores with every threshold.
In particular, they both achieve an almost perfect result (only one false positive, no false negatives) using the mean+std threshold.
The \texttt{paraphrase-multilingual-mpnet} model perform slightly worse than the monolingual version, providing encouraging results in the perspective of future multilingual applications.
The TF-IDF model is the one that performs worse with all the threshold values, in part probably due to the small size of the vocabulary.

Table~\ref{table:matches} shows an example of matching using sentences from S1 to S19, which are the one related to the argumentative nodes ``Has celiac disease", ``Has not celiac disease", ``Is immunosuppressed", ``Is not immunosuppressed".
The matches are computed by the \texttt{stsb-mpnet} and the \texttt{paraphrase-mpnet} models using a threshold value of 0.65.
The former achieves perfect precision but not perfect recall, and indeed we can see that it misses some matches, such as S8 and S10.
The latter reaches perfect recall but not precision, which indicates the presence of false positives e.g. the pair S1 and S8.
%
Some of these false positives might be particularly dangerous in a real application since they mean that the system has misunderstood a sentence for its negation, e.g. the sentence "I am not celiac" as "I am celiac".
The argumentative reasoning module would be able to detect such conflicts and in future works we plan to include conflict resolution modules and procedures. A careful user experience design may also be able to mitigate the issue, for instance by displaying relevant pieces of information interactively as they are understood by the system.


\begin{table}[!t]
\centering
 \caption{Matches computed by the models using the 0.65 threshold value on sentences from S1 to S19.  The $+$ symbol indicates the correct matches. The $\bullet$ symbol indicates the matches computed using the \texttt{stsb-mpnet model}. The $\circ$ symbol indicates the matches computed using the \texttt{paraphrase-mpnet} model.}
 \label{table:matches}
 \begin{tabular}{|c||c|c|c|c|c|c||c|c|c|c||c|c|c||c|c|c|c|c|c|}
 \hline
% \noalign{\smallskip}
    & S1 & S2 & S3 & S4 & S5 & S6 & S7 & S8 & S9 & S10 & S11 & S12 & S13 & S14 & S15 & S16 & S17 & S18 & S19 \\
 \hline\hline
	S1 & $+_{\bullet}^{\circ}$  &  $+_{\bullet}^{\circ}$ &  $+_{\bullet}^{\circ}$ &  $+_{\bullet}^{\circ}$ &  $+_{\bullet}^{\circ}$ & $+_{\bullet}^{\circ}$  & & ${^{\circ}}$ & & & & & & & & & & & \\
 \hline
	S2 & $+_{\bullet}^{\circ}$ &  $+_{\bullet}^{\circ}$ &  $+_{\bullet}^{\circ}$ &  $+_{\bullet}^{\circ}$ &  $+_{\bullet}^{\circ}$ & $+_{\bullet}^{\circ}$  & & & & & & & & & & & & & \\
 \hline
	S3 & $+_{\bullet}^{\circ}$ &  $+_{\bullet}^{\circ}$ &  $+_{\bullet}^{\circ}$ &  $+_{\bullet}^{\circ}$ &  $+_{\bullet}^{\circ}$ & $+_{\bullet}^{\circ}$  & & & & & & & & & & & & & \\
 \hline
	S4 &  $+_{\bullet}^{\circ}$ &  $+_{\bullet}^{\circ}$ &  $+_{\bullet}^{\circ}$ &  $+_{\bullet}^{\circ}$ &  $+_{\bullet}^{\circ}$ & $+_{\bullet}^{\circ}$  & ${^{\circ}}$ & & & & & & & & & & & & \\
 \hline
	S5 &  $+_{\bullet}^{\circ}$ &  $+_{\bullet}^{\circ}$ &  $+_{\bullet}^{\circ}$ &  $+_{\bullet}^{\circ}$ &  $+_{\bullet}^{\circ}$ & $+_{\bullet}^{\circ}$  & & & & & & & & & & & & & \\
 \hline
	S6 &  $+_{\bullet}^{\circ}$ &  $+_{\bullet}^{\circ}$ &  $+_{\bullet}^{\circ}$ &  $+_{\bullet}^{\circ}$ &  $+_{\bullet}^{\circ}$ & $+_{\bullet}^{\circ}$  & & & & & & & & & & & & & \\
 \hline
 \hline
    S7  & & & & ${^{\circ}}$ & & & $+_{\bullet}^{\circ}$ & $+_{\bullet}^{\circ}$ & $+_{\bullet}^{\circ}$ & $+_{\bullet}^{\circ}$ & & & & & & & & & \\
 \hline
	S8   & ${^{\circ}}$ & & & & & & $+_{\bullet}^{\circ}$ & $+_{\bullet}^{\circ}$ & $+_{\bullet}^{\circ}$ & $+_{}^{\circ}$ & & & & & & & & & \\
 \hline
	S9   & & & & & & & $+_{\bullet}^{\circ}$ & $+_{\bullet}^{\circ}$ & $+_{\bullet}^{\circ}$ & $+_{\bullet}^{\circ}$ & & & & & & & & & \\
 \hline
	S10   & & & & & & & $+_{\bullet}^{\circ}$ & $+_{}^{\circ}$ & $+_{\bullet}^{\circ}$ & $+_{\bullet}^{\circ}$ & & & & & & & & & \\
 \hline
 \hline
	S11 & & & & & & & & & & & $+_{\bullet}^{\circ}$ & $+_{\bullet}^{\circ}$ & $+_{}^{\circ}$ & ${^{\circ}}$ & & & & & \\
 \hline
	S12 & & & & & & & & & & & $+_{\bullet}^{\circ}$ & $+_{\bullet}^{\circ}$ & $+_{\bullet}^{\circ}$ & & & & & & \\
 \hline
	S13 & & & & & & & & & & & $+_{}^{\circ}$ & $+_{\bullet}^{\circ}$ & $+_{\bullet}^{\circ}$ & & & & & & \\
 \hline
 \hline
	S14 & & & & & & & & & & & ${^{\circ}}$ &  & & $+_{\bullet}^{\circ}$ & $+_{\bullet}^{\circ}$ & $+_{\bullet}^{\circ}$  & $+_{\bullet}^{\circ}$ & $+_{\bullet}^{\circ}$ & $+_{\bullet}^{\circ}$ \\
 \hline
	S15 & & & & & & & & & & & & & & $+_{\bullet}^{\circ}$ & $+_{\bullet}^{\circ}$ & $+_{\bullet}^{\circ}$  & $+_{\bullet}^{\circ}$ & $+_{\bullet}^{\circ}$ & $+_{\bullet}^{\circ}$ \\
 \hline
	S16 & & & & & & & & & & & & & & $+_{\bullet}^{\circ}$ & $+_{\bullet}^{\circ}$ & $+_{\bullet}^{\circ}$  & $+_{\bullet}^{\circ}$ & $+_{\bullet}^{\circ}$ & $+_{\bullet}^{\circ}$ \\
 \hline
	S17 & & & & & & & & & & & & & & $+_{\bullet}^{\circ}$ & $+_{\bullet}^{\circ}$ & $+_{\bullet}^{\circ}$  & $+_{\bullet}^{\circ}$ & $+_{\bullet}^{\circ}$ & $+_{\bullet}^{\circ}$ \\
 \hline
	S18 & & & & & & & & & & & & & & $+_{\bullet}^{\circ}$ & $+_{\bullet}^{\circ}$ & $+_{\bullet}^{\circ}$  & $+_{\bullet}^{\circ}$ & $+_{\bullet}^{\circ}$ & $+_{\bullet}^{\circ}$ \\
 \hline
	S19 & & & & & & & & & & & & & & $+_{\bullet}^{\circ}$ & $+_{\bullet}^{\circ}$ & $+_{\bullet}^{\circ}$  & $+_{\bullet}^{\circ}$ & $+_{\bullet}^{\circ}$ & $+_{\bullet}^{\circ}$ \\
 \hline

 \end{tabular}
\end{table}

These results are encouraging and motivate us to continue along this research direction. Nonetheless, our research is still in its early stages and that we are aware that a proper and sound evaluation of the whole proposal would require to include more nodes, a rigorous split between calibration and test sentences, and should eventually be validated by human testers.
